KLEESPECTRE: Detecting Information Leakage through Speculative Cache Attacks via Symbolic Execution

Spectre attacks disclosed in early 2018 expose data leakage scenarios via cache side channels. Specifically, speculatively executed paths due to branch mis-prediction may bring secret data into the cache which are then exposed via cache side channels even after the speculative execution is squashed. Symbolic execution is a well-known test generation method to cover program paths at the level of the application software. In this paper, we extend symbolic execution with modelingof cache and speculative execution. Our tool KLEESPECTRE, built on top of the KLEE symbolic execution engine, can thus provide a testing engine to check for the data leakage through cache side-channel as shown via Spectre attacks. Our symbolic cache model can verify whether the sensitive data leakage due to speculative execution can be observed by an attacker at a given program point. Our experiments show that KLEESPECTREcan effectively detect data leakage along speculatively executed paths and our cache model can further make the leakage detection much more precise.

==> mainbody.tex <==
\section{Threat model}
\label{sec:tm}

Traditional threat model of cache side-channel attack \cite{liu2015last} assumes that the victim and the attacker coexist on a machine, and they share the hardware resources such as cache. The attacker can execute any code in its security domain (e.g. a process or a virtual machine) and it has the ability to learn information from the side-channel. Our threat model is similar to this model, but we do not make the limitation that victim has to reside along with the attacker, for example, the remote timing attack~\cite{schwarz2018netspectre}.

Moreover, we make the following assumption:
\begin {assumption} \label{as:all} 
	All condition branch $br \in P$ are vulnerable that all of them can be mis-trained by another process, where $P$ is a given program. 
\end {assumption}

This assumption is reasonable since CPU sees the branch instruction for the first time, the static prediction logic is used to determine whether the branch is taken \cite{maisuradzespeculose}, the attacker can pollute (flush or evict) the branch predictor to force the speculation to the default branch. This might cause mis-prediction. Besides, the Branch predictor is shared by the processes running on the same core and branch predictor uses the hash value of the virtual address to index the pattern history table (PHT), so it is possible that the branches from different processes share the same entry in PHT, if 
\[ hash(addr(br_{P_i})) =  hash(addr(br_{P_j})) \]
where $br_{P_i}$, $br_{P_j}$ are two branch instructions from process $P_i$, $P_j$, respectively. As a result, the attacker can train the branch prediction inside its process thus mis-train the branch in the victim's process. 


%\begin{figure}[h]
%\begin{Verbatim}[frame=single, fontsize=\footnotesize]
\begin{lstlisting} [basicstyle=\footnotesize\ttfamily, breaklines=true, language=c++, frame=single, numbers=left, caption={Example 1.}\label{lst:e1}, keywordstyle=\color{blue}]
int a=100, size=16; 
char array1[16];
char array2[256*64];
int victim() {
  int y=0, temp=0;  
  if (a < size) {   //CB
    y = array1[a];
    temp |= array2[y];
  }   
  return temp;
}
\end{lstlisting}
%\end{Verbatim}

%\end{figure}
%\caption {Example 1.}
%\label {e1}


Consider the code in listing~\ref{lst:e1}, the conditional branch  in line 6 cannot be satisfied, it means the code in line 7, 8 will never be executed without speculation. However, based on the assumption~\ref {as:all}, the code in line 7 and 8 can leak 1 byte data if the branch in line 6 is mis-trained. Note that, the branch and the memory access in line 7 does not rely on the input. 

%\section{Threat model of oo7}
%Traditional threat model of access-based cache side-channel attack \cite{liu2015last} assumes that the victim and the attacker coexist on a machine, and they share the hardware resources such as cache. The attacker can execute any code in its security domain (e.g. a process or a virtual machine) and it has ability to learn knowledge from the covert channel. Our threat model is similar to this model, but we do not restraint that victim has to reside along with the attacker, the remote attack \cite{schwarz2018netspectre} which performs the timing-based attack is also adaptable in our threat model. Besides, we make more assumptions about the victim and attacker: 
%
%\begin{enumerate}
%	\item The victim does not contains any code that vulnerable to the general overflow attack, in other words, the victim's code is carefully checked and all memory accesses are well bounded. 
%	\item The vulnerable branches in victim's code can be indirectly controlled by attacker. The attacker train the branches by feeding delicately constructed data to the victim via network or other inter-precess communications. 
%\end{enumerate}


\section {Analysis of false negative / positive} 

\begin{figure}
	\centering
	\includegraphics[width=0.9\linewidth]{./fig/modules.png}
	\caption{Modules used in speculative symbolic execution modeling.}
	\vspace*{-0.1in}
	\label{fig:modules}
\end{figure}

Figure~\ref{fig:modules} lists four modules that will be used in the speculative execution modeling: static program analysis profiles the program to find the potential vulnerable paths for guiding the symbolic execution; Symbolic execution engine performs the symbolic execution; Speculative execution modeling works on symbolic execution engine and models the speculative execution; Cache modeling simulates the cache to further verify whether the data can be leaked in cache state for the different attack models. The analysis of false negative / positive (FN / FP)will based on the theses modules.

\subsection {FN / FP of static program analysis. }
Since symbolic executing all feasible program paths does not scale to large program, preprocessing of the program can provide some path information to guide the symbolic execution only working on the potential vulnerable paths can significantly improve the scalability of symbolic execution. 

\begin{enumerate}
	\item \textbf{False negative} For practice purpose, the static analysis cannot be sound, since the code features such as dynamically generated code, code reflection cannot be analyzed in static analysis. Therefore, the static analysis always contains false negatives, but it is acceptable and acknowledged.
	\item \textbf{False positive} Static analysis in this project just provide rough result for the latter symbolic execution, it is always computed in an over-approximation way. Hence the output of static analysis might result in false positives. 
\end{enumerate}

\subsection{FN / FP of symbolic execution}
\begin{enumerate}
	\item \textbf{False negative} The path explosion problem of symbolic execution might not allows the analysis traversing all paths due to the time constraint, and the improper selection of loop bound may introduce the false negatives.
	\item \textbf{False positive} If the constraints for a conditional branch cannot be solved in a given time, the engine will go to both directions of the branches. This might bring the false positives since the data leakage may be found in the unreachable paths. 
\end{enumerate}

\subsection {FN / FP of speculative execution modeling}
As mentioned in the section~\ref{sec:tm}, our analysis will consider all conditional branches as vulnerable. The speculative execution will be modeled at all conditional branches and thus there should not be any false negatives. 

The modeling of speculative execution window (SEW) is an over-approximation. Since SEW is the largest number of instructions that can be potentially  speculatively executed, the real speculative execution may not execute all of them. The over-approximation of SEW may introduce false positives. 

%The detected vulnerability might not leak the secret. Since we assume all input as secret, the out-of-bound memory access may not reach the real secret. 


%\subsection {FN / FP of cache modeling}


%\subsection {FN / FP of vulnerability detection}

\begin{figure*}[ht]
	\centering
	\includegraphics[width=0.95\linewidth]{./fig/cache.pdf}
	\caption{An example of cache modeling. A 2-way cache with 2 cache sets is used in this example. The symbols $c_i$ and $s_i$ denote the concrete and symbolic memory accesses, respectively. The red cross marks show where a cache line eviction happens.}
	\label{fig:cache}
\end{figure*}

\section {Methodology}
\subsection {Notation of symbolic execution}
In the traditional symbolic execution, a symbolic execution engine maintains a set of states. Each state $S$ determines the execution state at any execution point and the state can be represented as:

 \begin{equation}
 S = \langle pc, \delta, \pi \rangle
 \end{equation} 
where $pc$ is the next statement the engine will execute, and $\delta$ is a set of symbolic variables and each of them is represented as an expression $\alpha_i$. Each expression can be a constant value $const(\alpha_i)$ or a symbolic value $symb(\alpha_i)$. Moreover, $\pi$ is a formula that expresses a collection of constraints on symbols $\alpha_i$ due to branches taken in the execution to reach $pc$. 

 
%\subsection{Notation of speculative execution}

%\subsection{The state forks}

\section {Cache model}
The cache model in Worst Case Execution Time (WCET) analysis concerns the timing predictability and it tries to determine the worst execution time by figuring out the exact number of the cache misses and hits. Different from the cache model in WCET analysis, our cache model checks whether a set of sensitive addresses possibly remain in the cache at a given program point $P_s$. Specifically, the trace-based cache side-channel attack model assumes an attacker can probe the cache after each program point $P_s$, while the access-based attack model makes the assumption that an attacker can only probe the cache after the termination of the victim program $P_T$. Therefore, Our cache model is like the $may$-cache in WCET analysis \cite{reineke2007timing}. The safest $may$-cache should contain every memory block that appears on an execution path that may be mapped to the particular cache set. Our cache design should be an over-approximate one that only performs deterministic eviction leaving all other memory blocks in the cache.

Let us consider a memory block $m$ with a symbolic address $addr(m)$. It possibly maps to multiple cache sets, and for each cache set where $m$ may map, it will definitely be evicted from cache after a sequence of memory accesses with concrete addresses, if the memory accesses can certainly fill up a cache set. Based on this observation, our basic idea is that if the memory block $m$ has a symbolic address, we put the memory block $m$ to all cache sets where it may map and we only perform the eviction of $m$ after the cache set is filled up by the memory blocks which has a concrete address. 

Figure~\ref{fig:cache} shows an example of our cache modeling. The cache is initialized by the concrete memory accesses $c_1, c_2$ and $c_3$ where $c_1$ and $c_2$ map to cache set $0$ and $c_3$ maps to cache set $1$ in the phase (1). A symbolic memory access $s_1$ comes in phase (2). Since $s_1$ is symbolic, it may map to all cache sets, so it is placed in the virtual way $v-way$ of both cache set $0$ and set $1$ with a life tag 2 in the bracket. $s_1$ does not evict $c_1$ in the concrete cache line because $s_1$ is a $MAY$ mapping and we only evict the cache line when it is a deterministic operation. Then a concrete memory access $c_4$ comes into set $1$ in phase (3), and it reduces the life tag of $s_1$ in set $1$ from 2 to 1. In phase (4), $s2$ comes and maps to both cache sets $0$ and $1$. It also does not evict any cache line, since it is a $MAY$ mapping. After $c_5$ comes into set $0$ in phase (5), $c1$ is evicted from cache, at the same time, the life tag of $s_1$ and $s_2$ are reduced from 2 to 1. $c_6$ in phase (6) evicts $c_2$ and reduces the life tag of $s_1$ and $s_2$ to 0, so $s_1$ and $s_2$ are removed from the virtual cache line of set $0$. Then $c_7$ comes at phase (7), $c3$ and $s_1$ are removed from the cache set $1$. Finally, only $c_5, c_6, c_7, c_4$ and a symbolic $s_1$ remain in the cache. If any memory block in the final cache state has a sensitive memory address that may leak the secret and it is vulnerable to the Spectre attack.    
   
We add the cache state $\epsilon$ to the execution state $S$ to denote that at any execution point, there exists a unique cache state $\epsilon$: 
\begin{equation}
 S = \langle pc, \delta, \pi, \epsilon \rangle
\end{equation}

The cache state $\epsilon$ can be updated after a memory access with address $addr$ is described by the update function:
\begin{equation}
 \epsilon \times addr \rightarrow \epsilon
\end{equation}

Note that both the load and store operations on the normal execution path can update the cache, but on the speculative execution, only the load operation can update the cache state. This is because the store operation on the speculative execution path is not visible to the cache due to the assumption that all speculative executions are caused by the mis-prediction and that all stores will be rolled back after the branch is resolved.   

The cache is represented by the triple $<2^S, 2^{\beta}, \mathcal{A}>$ where $2^S$, $2^{\beta}$ and $\mathcal{A}$ capture the number of cache sets, cache line size and the associativity, respectively. We consider the $\mathcal{A}$-way set associative cache as a sequence of sets $F=<f_0,...,f_{2^S-1}>$, a set $f_i$ as a sequence of set lines $L=<l_0,...,l_{\mathcal{A}-1}, l_v>$. Note that we add a virtual cache line $l_v$ in a cache set along with the normal cache lines $l_1,...l_{\mathcal{A}-1}$ to store the symbolic memory access which may map to this cache set. 
Moreover, the store as a set of memory blocks $M=\{m_1,...,m_s\}$. 
The cache set for a concrete memory access of block $m$ is calculated by:
\begin{equation}
 set(addr(m)) = (addr(m) / 2^{\beta})\% 2^S 
\end{equation}

Moreover, a symbolic memory access with the symbolic address may map to multiple cache sets. For checking whether a symbolic address $addr(m)$ can map to cache set $i$, we query the solver with the following constraints:
\[\pi \wedge set(addr(m)) = i \Rightarrow true \]

Where $\pi$ is the path constraints.
 

\begin{equation}
cs(m) = \begin{cases} 
          \{set(addr(m))\},\ if\ const(addr(m)) \\
          \bigcup\limits_{i=0}^{2^\beta} \{i | \pi \wedge set(addr(m)) = i \Rightarrow true \}, if\ symb(addr(m))
           \end{cases}
\end{equation}

The formula describes that if an address is a constant expression, it can only map to an unique cache set. In contrast, if an address is a symbolic expression, it may map to multiple cache sets (a set of cache set index). 

{\bf Cache line eviction.} We use $s(l_i)$ that returns a set of memory blocks map to cache line $l_i$. For a constant address, it can map to a certain cache set, the update function is represented as follows:
\begin{equation}
update(s, const(m)) = \begin{cases}
								[l_1 \mapsto m, \\
								 l_i \mapsto s(l_{i-1}) | i = 2...h, \\
								 l_i \mapsto s(l_i) | i = h+1 ... A]; if \exists l_h: s(l_h) = m \\
								 \\
								 [l_1 \mapsto m \\
								 l_i \mapsto s(l_{i-1})\ for i=2...A]; otherwise
								 
                        \end{cases}
\end{equation}

For a memory block $m$ with a symbolic address $symbolic(addr(m))$, we put $m$ to the virtual cache line with a life tag, the life tag is initialized to the cache associativity $\mathcal{A}$. The life tag reduces when there is a concrete cache miss, and the memory block in the virtual cache line will be removed if its life time is 0. The update function for arbitrary memory block is modeled as follow:
\begin{equation}
update(s, m) = \begin{cases}
[l_v \mapsto m \cup s(l_v), \\
 \mathcal{A} \Rightarrow life(m)];\ if\ symb(addr(m)) \\
\\
[update(\epsilon, const(m)), \\
life(m_i)-1 \Rightarrow life(m_i), \\
\forall m_i \in s(l_v)];\ if \nexists l_h:s(l_h) = m

\end{cases}
\end{equation}


